KonVid-150k: A Dataset for No-Reference Video Quality Assessment of Videos in-the-Wild

Video quality assessment (VQA) methods focus on particular degradation types, usually artificially induced on a small set of reference videos. Hence, most traditional VQA methods under-perform in-the-wild. Deep learning approaches have had limited success due to the small size and diversity of existing VQA datasets, either artificial or authentically distorted. We introduce a new in-the-wild VQA dataset that is substantially larger and diverse: KonVid-150k. It consists of a coarsely annotated set of 153,841 videos having five quality ratings each, and 1,596 videos with a minimum of 89 ratings each. Additionally, we propose new efficient VQA approaches (MLSP-VQA) relying on multi-level spatially pooled deep-features (MLSP). They are exceptionally well suited for training at scale, compared to deep transfer learning approaches. Our best method, MLSP-VQA-FF, improves the Spearman rank-order correlation coefficient (SRCC) performance metric on the commonly used KoNViD-1k in-the-wild benchmark dataset to 0.82. It surpasses the best existing deep-learning model (0.80 SRCC) and hand-crafted feature-based method (0.78 SRCC). We further investigate how alternative approaches perform under different levels of label noise, and dataset size, showing that MLSP-VQA-FF is the overall best method for videos in-the-wild. Finally, we show that the MLSP-VQA models trained on KonVid-150k sets the new state-of-the-art for cross-test performance on KoNViD-1k, LIVE-VQC, and LIVE-Qualcomm with a 0.83, 0.75, and 0.64 SRCC, respectively. For both KoNViD-1k and LIVE-VQC this inter-dataset testing outperforms intra-dataset experiments, showing excellent generalization.

==> tables/tab-vqadatabases.tex <==
\caption{Attributes of existing VQA databases. Our proposed databases (KonVid-150k, KonViD-1600) are displayed in bold.}
\label{tab:vqadatabases}
\centering
\begin{tabular}{| l | r | r | r | r | r | r |} 
\hline
Attribute / Database    & CVD2014   & LIVE-Q.   & KoNViD-1k     & LIVE-VQC      & \textbf{FlickrVid-150k-A}      & \textbf{FlickrVid-150k-B}  \\ \hline
Year                & 2016      & 2017      & 2017          & 2020          & 2020              & 2019          \\ \hline
Unique contents            & 5         & 54        & $\approx1200$ & $\approx585$  & $\approx150,000$   & 1600          \\ \hline
Stimuli             & 234       & 208       & 1200          & 585           & 153,841            & 1596          \\ \hline
Ratings per Video   & 27-33     & 39        & 50            & >200          & 5                 & 89-175        \\ \hline
Devices             & 78        & 8         & N/A           & 43            & $\approx4500$(?)* & (?)           \\ \hline
Duration            & 10-25     & 15        & 8             & 10            & 5                 & 5             \\ \hline
Resolution          & VGA/720p  & 1080p     & 540p          & various       & 540p              & 540p          \\ \hline
Frame Rate          & 10-31     & 30        & 30            & N/A           & 24-120            & 24-120        \\ \hline
Format              & various   &YUV        & MPEG-4        & N/A           & MPEG-4            & MPEG-4        \\ \hline %CVD: MPEG-4, H.264, DV
\end{tabular}
% \raggedright \\
% \tiny
% * Number of devices is estimated based on the number of unique video authors ($\approx$ one camera each). It is likely that multiple authors use the same camera model.
